Towards Runtime Verification via Event Stream Processing in Cloud Computing Infrastructures

Software bugs in cloud management systems often cause erratic behavior, hindering detection, and recovery of failures. As a consequence, the failures are not timely detected and notified, and can silently propagate through the system. To face these issues, we propose a lightweight approach to runtime verification, for monitoring and failure detection of cloud computing systems. We performed a preliminary evaluation of the proposed approach in the OpenStack cloud management platform, an "off-the-shelf" distributed system, showing that the approach can be applied with high failure detection coverage.

==> tex/multi-user_network.tex <==
The structure of network operation rules is more complex than those of the rules for volume operations and instance creation. Thus, we use three interconnected EPL statements for expressing each of these rules. In the single-user scenario, network operation rules aim to verify if the number of events of a certain type exceeds the maximum threshold, determined by analyzing fault-free traces. In the multi-user scenario, the maximum threshold becomes equal to the maximum threshold in the single-user case times the number of users.  Assuming that the number of users is unknown a priori, we estimate the number of users by counting the number of {\lmttfont <neutron-vo-SecurityGroupRule-1.0, push>}
 events. The counter {\lmttfont countEvent}) simulates a counter of the number of users since there is only a single {\lmttfont <neutron-vo-SecurityGroupRule-1.0, push>} event that belongs to any fault-free or faulty trace. In \ref{lst:multiuser_neutron}, we show an example of a multi-user EPL rule for network operation.
 
 \begin{lstlisting}[caption=EPL rule for network operation,label={lst:multiuser_neutron}]
@name('S1') insert into NetworkEventStream select *
from Event where name='q-plugin_release_dhcp_port';
@name('S2') insert into InfoStream select count(*) as count1, max(countEvent) as maxCnt from NetworkEventStream;
@name('NetworkRule#1') select  * from InfoStream where count1 > maxEvent*maxCnt
output when OutputTriggerVar = true
then set OutputTriggerVar = false;
\end{lstlisting}
 
 The first statement ({\lmttfont S1}) extracts {\lmttfont <q-plugin, release\_dhcp\_port>} events and inserts them in the stream {\lmttfont NetworkEventStream}. The second statement ({\lmttfont S2}) counts the number of events in {\lmttfont NetworkEventStream}, the maximum value of {\lmttfont countEvent}) of the events in {\lmttfont NetworkEventStream} and passes these pieces of information to the stream {\lmttfont InfoStream}, respectively as {\lmttfont count1} and {\lmttfont maxCnt}. Finally, the third statement ({\lmttfont NetworkRule#1}) produces an output if the {\lmttfont count1} value  in {\lmttfont InfoStream} is bigger than the maximum number of {\lmttfont <q-plugin, release\_dhcp\_port>} events in fault-free traces ({\lmttfont maxEvent}) times the estimated number of users/performed requests ({\lmttfont maxCnt}). To avoid that the third statement outputs anytime it receives a new {\lmttfont <q-plugin, release\_dhcp\_port>} event after the first output, we use the {\lmttfont OutputTriggerVar} boolean variable, initialized to true and set to false after the first time the rule is verified. 
